H-InDex: Visual Reinforcement Learning with Hand-Informed Representations for Dexterous Manipulation

Human hands possess remarkable dexterity and have long served as a source of inspiration for robotic manipulation. In this work, we propose a human $\textbf{H}$and$\textbf{-In}$formed visual representation learning framework to solve difficult $\textbf{Dex}$terous manipulation tasks ($\textbf{H-InDex}$) with reinforcement learning. Our framework consists of three stages: (i) pre-training representations with 3D human hand pose estimation, (ii) offline adapting representations with self-supervised keypoint detection, and (iii) reinforcement learning with exponential moving average BatchNorm. The last two stages only modify $0.36\%$ parameters of the pre-trained representation in total, ensuring the knowledge from pre-training is maintained to the full extent. We empirically study 12 challenging dexterous manipulation tasks and find that H-InDex largely surpasses strong baseline methods and the recent visual foundation models for motor control. Code is available at https://yanjieze.com/H-InDex .

==> trash.tex <==
\begin{table}[H]
\caption{\textbf{Episode returns for main experiments.} Highest returns for each task are marked with \textbf{bold} fonts. }
\label{tab:episode returns}
\vspace{0.05in}
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{cccccc}
\toprule
Task name / Method & RRL~\cite{shah2021rrl} & R3M~\cite{nair2022r3m} & MVP~\cite{xiao2022mvp} & VC-1~\cite{majumdar2023vc1} &  \ours \\ \midrule
\texttt{Hammer} &
\dd{8793}{2475} &
\dd{1753}{1780} &
\dd{10052}{1282} &
\dd{12503}{226} &
\ddbf{16373}{187} \\

\texttt{Door} &
\dd{2469}{294} &
\dd{2885}{82} &
\ddbf{2933}{41} &
\dd{2878}{109} &
\dd{2837}{39} \\

\texttt{Pen} &
\dd{2936}{149} &
\dd{2082}{129} &
\dd{3309}{98} &
\dd{3341}{108} &
\ddbf{3589}{185} \\

\texttt{Pour} &
\dd{12074}{1790} &
\dd{36}{14} &
\dd{14596}{3368} &
\dd{17141}{2651} &
\ddbf{19814}{802} \\


\texttt{Place inside} &
\dd{136}{111}&
\dd{1}{4}&
\dd{244}{8}&
\dd{198}{51}&
\ddbf{251}{7}\\

\texttt{Relocate large clamp} &
\dd{526}{357} &
\dd{132}{162} &
\dd{762}{93} &
\dd{762}{569} &
\ddbf{1046}{411} \\

\texttt{Relocate foam brick} &
\dd{1229}{230}&
\dd{629}{512}&
\dd{1048}{928}&
\dd{884}{995}&
\ddbf{1527}{9}
\\

\texttt{Relocate box} &
\dd{947}{613}&
\dd{565}{230}&
\dd{1142}{1154}&
\dd{800}{645}&
\ddbf{1241}{281}\\


\texttt{Relocate mug} &
\dd{1832}{333}&
\dd{1351}{114}&
\dd{1884}{1295}&
\ddbf{2390}{844}&
\dd{2270}{103}\\



\texttt{Relocate mustard bottle} &
\dd{1653}{50}&
\dd{935}{134}&
\dd{2249}{183}&
\ddbf{2262}{98}&
\dd{2092}{32}\\

\texttt{Relocate tomato soup can} &
\dd{1886}{412}&
\dd{422}{722}&
\dd{1071}{910}&
\dd{1020}{722}&
\ddbf{2105}{63}\\

\texttt{Relocate potted meat can} &
\dd{2215}{175}&
\dd{1033}{97}&
\dd{1776}{1391}&
\ddbf{2392}{603}&
\dd{2240}{85}\\

\texttt{Normalized Average} &
$72.8$&
$35.7$&
$80.1$&
$81.4$&
\cc{\textbf{98.2}}\\

\bottomrule
\end{tabular}
}
\end{table}
